On Designing Secure and Robust Scan Chain for Protecting Obfuscated Logic

In this paper, we assess the security and testability of the state-of-the-art design-for-security (DFS) architectures in the presence of scan-chain locking/obfuscation, a group of solution that has previously proposed to restrict unauthorized access to the scan chain. We discuss the key leakage vulnerability in the recently published prior-art DFS architectures. This leakage relies on the potential glitches in the DFS architecture that could lead the adversary to make a leakage condition in the circuit. Also, we demonstrate that the state-of-the-art DFS architectures impose some substantial architectural drawbacks that moderately affect both test flow and design constraints. We propose a new DFS architecture for building a secure scan chain architecture while addressing the potential of key leakage. The proposed architecture allows the designer to perform the structural test with no limitation, enabling an untrusted foundry to utilize the scan chain for manufacturing fault testing without needing to access the scan chain. Our proposed solution poses negligible limitation/overhead on the test flow, as well as the design criteria.

==> settings.tches.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2569-2925}
\makeatletter
\setDOI{10.13154/tches.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother

\setkeys{IACR}{journal=tches}


==> settings.tosc.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2519-173X}
\makeatletter
\setDOI{10.13154/tosc.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother

